Semantics and simulation of communication in quantum programming

We present the quantum programming language cQPL which is an extended version of QPL [P. Selinger, Math. Struct. in Comp. Sci. 14(4):527-586, 2004]. It is capable of quantum communication and it can be used to formulate all possible quantum algorithms. Additionally, it possesses a denotational semantics based on a partial order of superoperators and uses fixed points on a generalised Hilbert space to formalise (in addition to all standard features expected from a quantum programming language) the exchange of classical and quantum data between an arbitrary number of participants. Additionally, we present the implementation of a cQPL compiler which generates code for a quantum simulator.

==> erklaerung.tex <==
\thispagestyle{plain}
\chapter*{Erkl\"arung}
\selectlanguage{ngerman}
Gem\"a{\ss} \textsection 31(2) der \emph{Diplompr\"ufungsordnung 
f\"ur Studenten der Physik an der 
Fried\-rich-\hspace{0mm}Alexan\-der-Uni\-ver\-si\-t\"at 
Erlangen-N\"urnberg} vom \(20.08.2004\) versichere ich, dass ich 
die Arbeit selb\-st\"an\-dig ver\-fasst und keine anderen als die angegebenen
Quellen und Hilfsmittel benutzt habe.\par\vspace{2cm}

\noindent Erlangen, 26. Mai 2005\par\vspace{1.5cm}

\noindent\rule{3.5cm}{0.5pt}\\
\noindent Wolfgang Mauerer

